Dynamic N:M Fine-grained Structured Sparse Attention Mechanism

Transformers are becoming the mainstream solutions for various tasks like NLP and Computer vision. Despite their success, the high complexity of the attention mechanism hinders them from being applied to latency-sensitive tasks. Tremendous efforts have been made to alleviate this problem, and many of them successfully reduce the asymptotic complexity to linear. Nevertheless, most of them fail to achieve practical speedup over the original full attention under moderate sequence lengths and are unfriendly to finetuning. In this paper, we present DFSS, an attention mechanism that dynamically prunes the full attention weight matrix to N:M fine-grained structured sparse pattern. We provide both theoretical and empirical evidence that demonstrates DFSS is a good approximation of the full attention mechanism. We propose a dedicated CUDA kernel design that completely eliminates the dynamic pruning overhead and achieves speedups under arbitrary sequence length. We evaluate the 1:2 and 2:4 sparsity under different configurations and achieve 1.27~ 1.89x speedups over the full-attention mechanism. It only takes a couple of finetuning epochs from the pretrained model to achieve on par accuracy with full attention mechanism on tasks from various domains under different sequence lengths from 384 to 4096.

==> chapters/low_rank.tex <==
\section{Extension to Low-rank Transformer}

In this section, we demonstrate that our dynamic attention can also be applied to Low-rank transformers.

\subsection{Linformer}

The self-attention mechanism in Linformer is constructed as
\begin{equation}
    softmax\left(\frac{Q(EK)^T}{\sqrt{d}}\right)FV,
\end{equation}
Where $Q,K,V\in\mathbb{R}^{n\times d}$ are the query, key, and value. $E,F\in \mathbb{R}^{k\times n}$ are linear projection matrices learned during training. 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/linformer.jpeg}
    \caption{Sparse Linformer}
    \label{fig:data2meta}
\end{figure}

==> chapters/outline.tex <==
\section{Paper Outline}

Motivation
\begin{itemize}
    \item Transformer has high compute intensity \& memory footprint, the self-attention weight is the bottleneck under long sequence.
    \item The weight is very sparse (ref, exp), however, traditional static pruning is not applicable, as the attention weight is dynamic during inference.
    \item Existing studies that exploit the sparsity introduce nonnegligible overhead and the sparsity pattern is unfriendly to GPU. They usually failed to outperform dense GEMMs on high-end GPUs
    \item 50\% dropout is usually applied during training/fine-tuning.
\end{itemize}
Challenge
\begin{itemize}
    \item Difficult to efficiently obtain the dynamic sparse pattern
    \item Difficult to achieve speedup in SDDMM kernel
    \item Achieve practical speedup under moderate sparsity
\end{itemize}
Solution
\begin{itemize}
    \item Select important attention weights after SDDMM.
    \item Pattern: 50\% sparsity on Ampere GPU
    \item TODO: New 4-2 or 2-1 dropout (magnitude or random) , this may also be helpful during training.
    \item Kernel design: 0-overhead dynamic pruning
\end{itemize}

==> chapters/sparsity.tex <==
\section{Dynamic Sparse Transformer}

In order to generate a $2^m$ ticket pool with $k<m$ edges, instead of using a single fixed ticket pool, we can have a set of k-edge ticket pools. During the inference, a single k-edge ticket pool that is more likely to contain the wining ticket is selected. The overall cost (computational cost/memory footprint) equals to the cost of a k-edge ticket pool plus the pool selection cost. The effective pool size equals to the conjunction of the pools and selection probability.

Therefore, there are two criterions. 
\begin{itemize}
    \item Need high enough select Probability
    \item Need low enough overhead
    \item Need good speedup with k-edge ticket pool
\end{itemize}

Strength of our method
\begin{itemize}
    \item 100\% prediction accuracy
    \item zero overhead
    \item good speedup
\end{itemize}


\todo{-----------------------------}

: i.e. it changes accordingly to the input sequence.

\todo{-----------------------------}

\todo{existing dynamic sparse transformer cannot achieve practical speedup over dense counterpart}



\todo{-----------------------------}

\begin{itemize}
    \item Fixed attention + dynamic attention
    \item Speedup mainly from fixed attention, dynamic attention makes it slower
\end{itemize}

\textbf{50\% Structured dynamic sparsity}. Under \textit{float32}, the larger one is selected from consecutive two edges. We have $k=\frac{m}{log_23}\approx 0.63m$. 

Under \textit{bfloat16}, two larger ones are selected from consecutive four edges. We have $k=\frac{2m}{log_211}\approx 0.58m$

Therefore, we only need around 60\% edges.

\subsection{Fine-tuning Strategy}
Given a model pretrained under float data type, we can fine-tune it to recover the accuracy loss caused by the dynamic sparsity.

Under float data type, we need to adjust the model to fit the dynamic sparsity pattern. We choose to fine-tune from the base model (e.g. bert-large) instead of the model already tuned for specific tasks. This allows us to use higher learning rate to quickly adapt the model to the new attention pattern. 

When tuning the baseline model under bfloat16, we observe that the accuracy is poor if we directly tune from the base model. 

\todo{-----------------------------}

